Reinforcement Learning with Augmented Data

Learning from visual observations is a fundamental yet challenging problem in Reinforcement Learning (RL). Although algorithmic advances combined with convolutional neural networks have proved to be a recipe for success, current methods are still lacking on two fronts: (a) data-efficiency of learning and (b) generalization to new environments. To this end, we present Reinforcement Learning with Augmented Data (RAD), a simple plug-and-play module that can enhance most RL algorithms. We perform the first extensive study of general data augmentations for RL on both pixel-based and state-based inputs, and introduce two new data augmentations - random translate and random amplitude scale. We show that augmentations such as random translate, crop, color jitter, patch cutout, random convolutions, and amplitude scale can enable simple RL algorithms to outperform complex state-of-the-art methods across common benchmarks. RAD sets a new state-of-the-art in terms of data-efficiency and final performance on the DeepMind Control Suite benchmark for pixel-based control as well as OpenAI Gym benchmark for state-based control. We further demonstrate that RAD significantly improves test-time generalization over existing methods on several OpenAI ProcGen benchmarks. Our RAD module and training code are available at https://www.github.com/MishaLaskin/rad.

==> background.tex <==
%auto-ignore
\section{Background}

RL agents act within a Markov Decision Process, defined as the tuple $(\mathcal{S},\mathcal{A},P,\gamma)$, with the following components: states $s\in \mathcal{S}=\mathbb{R}^n$, actions $a\in \mathcal{A}$ either discrete ($\mathcal{A}=\mathbb{J}$) or continuous ($\mathcal{A}=\mathbb{R}^m$), and state transition probability function, $P=P(s_{t+1},r_t|s_t,a_t)$, which defines the task mechanics and rewards. Without prior knowledge of $P$, the RL agent's goal is to use experience to maximize expected rewards, $R=\sum_{t=0}^\infty \gamma^t r_t$, under discount factor $\gamma\in[0,1)$.  Crucially, in RL from pixels, the agent receives image-based observations, $o_t=O(s_t)\in \mathbb{R}^k$, which are a high-dimensional, indirect representation of the state. 
%The agents to learn to extract meaningful information from the observations.

\textbf{Soft Actor-Critic}. SAC~\cite{haarnoja2018soft} is a state-of-the-art off-policy algorithm for continuous control problems. SAC learns a policy, $\pi_\psi(a|o)$, and a critic, $Q_\phi(o,a)$, and aims to maximize a weighted objective of the reward and the policy entropy, $\mathbb{E}_{s_t,a_t\sim\pi} \left[\sum_t r_t + \alpha \mathcal{H}(\pi(\cdot|o_t))\right]$.  The critic parameters are learned by minimizing the squared Bellman error using transitions, $\tau_t=(o_t,a_t,o_{t+1},r_t)$, replayed from an experience buffer, $\mathcal{D}$:
\begin{equation}
    \label{eq:SAC_Q_Loss}
    \mathcal{L}_Q(\phi)=\mathbb{E}_{\tau\sim\mathcal{D}}\left[\big(Q_\phi(o_t,a_t) - (r_t + \gamma V(o_{t+1}))\big)^2\right].
\end{equation}
The target value of the next state can be estimated by sampling an action using the current policy:
\begin{equation}
    V(o_{t+1})=\mathbb{E}_{a'\sim\pi}\left[Q_{\tilde{\phi}}(o_{t+1},a')-\alpha \log\pi_\psi(a'|o_{t+1})\right],
\end{equation}
where $Q_{\tilde{\phi}}$ represents a more slowly updated copy of the critic.  The policy is learned by minimizing the divergence from the exponential of the soft-Q function at the same states:
\begin{equation}
    \label{eq:SAC_pi_Loss}
    \mathcal{L}_\pi(\psi)=-\mathbb{E}_{a\sim\pi}\left[Q_\phi(o_t,a)-\alpha \log\pi_\psi(a|o_t)\right],
\end{equation}
via the reparameterization trick for the newly sampled action. $\alpha$ is learned against a target entropy.
%, and a pair of critics and use their elementwise-minimum in the learning targets~\cite{fujimoto2018td3} for improved stability.  

\textbf{Proximal policy optimization}. PPO~\cite{schulman2017ppo} is a state-of-the-art on-policy algorithm for learning a continuous or discrete control policy, $\pi_\theta(a|o)$.  PPO forms policy gradients using action-advantages, $A_t=A^\pi(a_t,s_t)=Q^\pi(a_t,s_t)-V^\pi(s_t)$, and minimizes a clipped-ratio loss over minibatches of recent experience (collected under $\pi_{\theta_{old}}$):
\begin{equation}
    \label{eq:PPO_pi_Loss}
    \mathcal{L}_{\pi}(\theta)=-\mathbb{E}_{\tau\sim\pi}\left[\min\left(\rho_t(\theta) A_t, \ \text{clip}(\rho_t(\theta),1-\epsilon,1+\epsilon)A_t\right)\right], \quad \rho_t(\theta)=\frac{\pi_\theta(a_t|o_t)}{\pi_{\theta_{old}} (a_t|o_t)}.
\end{equation}
Our PPO agents learn a state-value estimator, $V_\phi(s)$, which is regressed against a target of discounted returns and used with Generalized Advantage Estimation~\cite{schulman2017ppo}:
\begin{equation}
    \label{eq:PPO_V_Loss}
    \mathcal{L}_V(\phi) = \mathbb{E}_{\tau\sim\pi}\left[\left(V_\phi(o_t)-V^{targ}_t\right)^2\right].
\end{equation}

\textbf{RAD}. When applying RAD to SAC, our data augmentations are applied to the observation passed to $Q$ in (\ref{eq:SAC_Q_Loss}) and $\pi$ in (\ref{eq:SAC_pi_Loss}).  Every use of the observation in (\ref{eq:PPO_pi_Loss})-(\ref{eq:PPO_V_Loss}) for training the PPO agent is subject to the same augmentation. However, unlike SAC, we apply the data augmentation on samples collected from rollouts because PPO is an on-policy RL method.


==> backup.tex <==
\begin{table}[h]
\centering
\small
\begin{tabular}{l|cccc}
\toprule
& Cheetah & Walker  & Hopper & Ant  \\ 
\midrule
PETS & 
2288.4 $\pm$ 1019.0 &
282.5 $\pm$ 501.6 &
114.9 $\pm$ 621.0 & 
1165.5 $\pm$ 226.9 \\
POPLIN-A &
1562.8 $\pm$ 1136.7&
-105.0 $\pm$ 249.8&
202.5 $\pm$ 962.5 &
1148.4 $\pm$ 438.3 \\
POPLIN-P &
4235.0 $\pm$ 1133.0 &
597.0 $\pm$ 478.8 &
2055.2 $\pm$ 613.8 &
{\bf 2330.1 $\pm$ 320.9} \\
METRPO &
2283.7 $\pm$ 900.4&
-1609.3 $\pm$ 657.5&
1272.5 $\pm$ 500.9 &
282.2 $\pm$ 18.0 \\
TD3 &
3015.7 $\pm$ 969.8&
-516.4 $\pm$ 812.2&
1816.6 $\pm$ 994.8 &
870.1 $\pm$ 283.8  \\ \midrule
SAC & 
4035.7 $\pm$ 268.0 &
-382.5 $\pm$ 849.5 &
2020.6 $\pm$ 692.9 &
836.5 $\pm$ 68.4 \\ 
SAC + BN &
3330.9 $\pm$ 508.4 &
{\bf 1025.5 $\pm$ 1256.2}& 
1860.1 $\pm$ 311.6 &
530.7 $\pm$ 110.6\\ \midrule
SAC + RAD (scalar-single)&
{\bf 4545.5 $\pm$ 1236.1} &
600.6 $\pm$ 955.4 & 
2110.7 $\pm$ 233.8 &
1019.9 $\pm$ 409.2 \\ 
SAC + RAD (scalar-multi)&
2788.8 $\pm$ 473.3&
{\bf 986.9 $\pm$ 498.3}& 
{\bf 2178.9 $\pm$ 431.2} &
1059.8 $\pm$ 282.2\\ 
SAC + RAD (Gaussian)&
1930.0 $\pm$ 623.6&
-114.1 $\pm$ 966.1& 
-66.0 $\pm$ 608.1 &
935.4 $\pm$ 18.4 \\ \midrule
Timesteps
& 200000 & 200000 & 200000 & 200000\\ \toprule
& Pendulum & Cartpole  & Acrobot  \\ 
\midrule
PETS & 
155.7 $\pm$ 79.3 &
199.6 $\pm$ 4.6 &
-18.4 $\pm$ 46.3  \\
POPLIN-A &
{\bf 178.3 $\pm$ 19.3} &
{\bf 200.6 $\pm$ 1.3} &
20.5 $\pm$ 20.1  \\
POPLIN-P &
167.9 $\pm$ 45.9 &
{\bf 200.8 $\pm$ 0.3}  &
{\bf 23.2 $\pm$ 27.2}  \\
METRPO &
174.8 $\pm$ 6.2 &
138.5 $\pm$ 63.2 &
-78.7 $\pm$ 5.0  \\
TD3 &
168.6 $\pm$ 12.7 &
-409.2 $\pm$ 928.8 &
-76.5 $\pm$ 10.2  \\\midrule
SAC & 
163.6$\pm$ 10.9 &
{\bf 200.5 $\pm$ 0.7} &
-71.8 $\pm$ 6.8   \\ 
SAC + BN &
157.7 $\pm$ 11.1 &
170.7 $\pm$ 51.6 &
-70.8 $\pm$ 6.2 \\ \midrule
SAC + RAD (random amplitude-s)&
166.9 $\pm$ 15.5 &
{\bf 200.0 $\pm$ 0.7} &
-69.3 $\pm$ 5.8  \\
SAC + RAD (random amplitude-m)&
167.3 $\pm$ 13.1 &
{\bf 200.0 $\pm$ 0.7} &
-77.6 $\pm$ 11.2  \\
SAC + RAD (Gau)&
157.5 $\pm$ 13.1 &
165.8 $\pm$ 45.1 &
-306.6 $\pm$ 112.8  \\ \midrule
Timesteps
& 50000 & 50000 & 50000 \\ \bottomrule
\end{tabular}
\vspace{0.1in}
\caption{The training time-step varies from 50,000 to 200,000 depending on the difficulty of the tasks.} 
\end{table}
